Can Adversarially Robust Learning Leverage Computational Hardness?

Making learners robust to adversarial perturbation at test time (i.e., evasion attacks) or training time (i.e., poisoning attacks) has emerged as a challenging task. It is known that for some natural settings, sublinear perturbations in the training phase or the testing phase can drastically decrease the quality of the predictions. These negative results, however, are information theoretic and only prove the existence of such successful adversarial perturbations. A natural question for these settings is whether or not we can make classifiers computationally robust to polynomial-time attacks. In this work, we prove strong barriers against achieving such envisioned computational robustness both for evasion and poisoning attacks. In particular, we show that if the test instances come from a product distribution (e.g., uniform over $\{0,1\}^n$ or $[0,1]^n$, or isotropic $n$-variate Gaussian) and that there is an initial constant error, then there exists a polynomial-time attack that finds adversarial examples of Hamming distance $O(\sqrt n)$. For poisoning attacks, we prove that for any learning algorithm with sample complexity $m$ and any efficiently computable "predicate" defining some "bad" property $B$ for the produced hypothesis (e.g., failing on a particular test) that happens with an initial constant probability, there exist polynomial-time online poisoning attacks that tamper with $O (\sqrt m)$ many examples, replace them with other correctly labeled examples, and increases the probability of the bad event $B$ to $\approx 1$. Both of our poisoning and evasion attacks are black-box in how they access their corresponding components of the system (i.e., the hypothesis, the concept, and the learning algorithm) and make no further assumptions about the classifier or the learning algorithm producing the classifier.

==> ConcMsr.tex <==
\section{Computational Concentration of Metric Probability Spaces}


==> GeneralRecepie.tex <==
\section{General Approach for Proving Computational Concentration}


\begin{definition}[McDiarmid Type inequality] 
\Mnote{we won't have the following form of inequalities in general, at least the way I tried to prove them in previous section. Maybe, you need $(c_1,c_2,c_3)$-Levy concentrated instead?}
A metric measure space $(\X, \msr, \metric)$ is $(c_1,c_2)$-concentrated if for any $\lambda$-Lipschitz measurable function $f:\X \to \R$ with average $a=\Ex_{x\gets \msr}[f(x)]$ we have 
$$\Pr[|f(x)-a| \geq \eps] \leq c_1\cdot \e^{-c_2 \eps^2/\lambda^2}$$
where $c_1$ and $c_2$ are constants. 
\end{definition}
\begin{definition} A metric measure space $(\X, \msr, \metric)$ has a $\lambda$-Lipschitz $\beta$-bounded $\delta$-dense  ($(\lambda,\beta,\delta)$-LBD for short) re-sampler, if there is a (re-sampling) randomized procedure $\CentDist\colon  \X \to \X$ such that the following hold:
\begin{itemize}
    \item {\bf $\lambda$-Lipschitz.} For any $x,x' \in \X$, we have $|\CentDist( x) - \CentDist( x')| \leq \lambda\cdot\metric(x,x')$ in statistical distance.
    
    \item {\bf $\beta$-bounded.} For any $x \in \X$, we have $\Pr_{x' \gets \CentDist( x)}[\metric(x,x')>\beta] = 0$.
        
    \item {\bf $\delta$-dense.} For any measurable set $\cS \se \X$, we have
    $$\Pr_{\substack{x\gets \msr\\ x'\gets \CentDist( x)}}[x' \in \cS] \geq \delta \cdot \msr(\cS).$$

\end{itemize}
\end{definition}

\begin{remark}[Connection to differential privacy]
The Lipschitz property is reminiscent of differential privacy, with the generalized metric substituting the Hamming distance used for comparing neighbor databases, and also statistical distance used instead of the stronger conditioned used in differential privacy condition. Also, the bounded property, at a high level, is related to the utility of the differentially  private mechanisms, as we want the re-sampled ``data base'' to be $\beta$-close to the original one.
\end{remark}

\begin{remark} Ideally, we prefer $(\lambda,\beta,\delta)$-LBD re-samplers with $\lambda \approx 0$, $\beta\approx 0$, and $\delta \approx 1$. If we don't care about the Lipschitz property, then we can trivially choose $\CentDist(x) = x$ that gives optimal $\beta = 0, \delta=1$. If we don't care about bounded property, we can trivially choose $\CentDist(x)\equiv \msr$ to be a fresh new sample, by which we get $\lambda=0, \delta =1$. However, if we don't care about $\delta$, it is not still clear how to get nontrivial $\lambda$ and $\beta$.
\end{remark}

\Mnote{need to update the theorem using $(c_1,c_2,c_3)$? also better to have a more general theorem for any concentrated space first (just like how we did it for previous paper) and then apply it to Levy.}\Snote{I still think there should be a way to parametrize the inequality with two variables. But I think we should go with three variables for now.}
\Snote{One thing that we can do is to stick to median. At the end we argue that median will be high when the average is high.}
\begin{theorem}
Let $(\X, \msr, \metric)$ be a $(c_1,c_2)$-concentrated metric measure space and let $\cS$ be a subset of the metric space with measure $h$. Also let $\CentDist$ be the $(\lambda,\beta,\delta)$-LBD re-sampler for this metric measure space. Then, there is an algorithm $A$ that given $x \in \X$, calls sampler $\CentDist$, $\poly(\frac{1}{h\cdot\delta})$ times and outputs $A(x)\in \X$ such that
$$\Pr_{\substack{x\gets \msr\\ x'\gets A(x)}}[x'\in \cS \wedge \metric(x,x')\leq \beta] \geq 1-c_1\cdot \e^{-c_2 \cdot h^2 \frac{\delta^2}{4\cdot\lambda^2}}.$$
\end{theorem}
\begin{proof}
$$f(x) = \Pr[\CentDist(x)\in \cS]$$
$$|f(x)-f(x')|\leq |\CentDist(x) -\CentDist(x')| \leq \lambda\cdot\metric(x,x')$$
$$h'=\Ex_{x\gets \msr}[f(x)] = \Pr_{\substack{x\gets \msr\\ x'\gets \CentDist(x)}} [x' \in \cS] \geq h\cdot \delta$$
$$\Pr [h' -f(x) \geq \frac{h'}{2}] \leq c_1\cdot \e^{-c_2 \frac{h'^2}{4\cdot\lambda^2}} \leq c_1\cdot \e^{-c_2 \cdot h^2 \frac{\delta^2}{4\cdot\lambda^2}}$$
$$\Pr [f(x) \leq \frac{\delta\cdot h}{2} ] \leq c_1\cdot \e^{-c_2 \cdot h^2 \frac{\delta^2}{4\cdot\lambda^2}}$$
\end{proof}


==> PrelimSTOC.tex <==
\section{Preliminaries} \label{sec:prelim}

\begin{definition}[Notation for metric  spaces]
Let $(\X,\metric)$ be a metric space. We use the notation
$\diam^\metric(\X) = \sup\set{\metric(x,y) \mid x,y \in \X_i}$ to denote the diameter of $\X$ under $\metric$, and we use $\Ball_b^\metric(x)=\set{x' \mid \metric(x,x') \leq b}$ to denote the ball of radius $b$ centered at $x$. We also use $\Sph_b^\metric(x)=\set{x' \mid \metric(x,x') = b}$ to denote the sphere of radius $b$ centered at $x$. \Mnote{how is sphere different from ball? by sphere you mean distance exactly b?}  When $\metric$ is clear from the context, we simply write $\diam (\X)$ and $\Ball_b (x)$. For a set $\cS\se \X$, by $\metric(x,\cS) = \inf\set{\metric(x,y) \mid  y \in \cS}$  we denote the distance of a point $x$ from $\cS$. 
\end{definition}

Unless stated otherwise, all integrals in this work  are Lebesgue integrals.

\begin{definition}[Nice metric probability spaces] \label{def:niceProb}
We call $(\X, \metric, \msr)$ a metric probability space, if  $\msr$ is a Borel probability measure over $\X$ with respect to the topology defined by $\metric$. Then, for a Borel set $\cE \se \X$, the \emph{$b$-expansion} of $\cE$, denoted by $\cE_b$, is defined as\footnote{The set $\cE_b$ is also called the $b$-flattening or $b$-enlargement of $\cE$, or simply the $b$-ball around $A$.} 
$$\cE_b = \set{x \mid \metric(x,\cE) \leq b}.$$ 
We call $(\X, \metric, \msr)$ a \emph{nice} metric probability space, if the following conditions hold.
\begin{enumerate}
    \item {\bf Expansions are measurable.} For every $\msr$-measurable (Borel) set $\cE \in \cX$, and every $b\geq 0$, its $b$-expansion  $\cE_b$ is also $\msr$-measurable. 
    \item {\bf Average distances exist.} For every two Borel sets $\cE,\cS \in \cX$, the average minimum distance of an element from $\cS$ to $\cE$ exists; namely, the integral $\int_\cS \metric(x,\cE) \cdot d\msr(x)$ exists. 
\end{enumerate}
\end{definition}



\subsection{Classification Problems}
\paragraph{Notation on learning problems.}  We  use calligraphic letters (e.g., $\cX$) for sets. 
By $x \gets \msr$ we denote sampling $x$  from the probability measure $\msr$. 
For a randomized algorithm $R(\cdot)$, by $y \gets R(x)$ we denote the randomized execution of $R$ on input $x$ outputting $y$. 
%By $\Supp(D) = \set{d \mid \Pr[D=d]>0}$ we denote the support set of $D$.  
 A classification problem $(\X,\Y,\msr,\C,\H)$ is specified by the following components. 
The set $\X$ is the set  of possible \emph{instances}, %and  
$\Y$ is the set of possible \emph{labels}, %and
$\msr$ is a distribution over $\X$,
$\C$ is a class of \emph{concept} functions where $c\in \C$ is always a mapping from $\X$ to $\Y$.
We did not state the loss function explicitly, as we work with classification problems.
 For  $x \in \X, c \in \C$,
the \emph{risk} or \emph{error} of a hypothesis $h \in \H$ is equal to $\Risk(h,c) = \Pr_{x \gets\msr}[h(x) \neq c(x)]$. We are usually interested in learning problems $(\X,\Y,\msr,\C,\H)$ with a specific metric $\metric$ defined over $\X$ for the purpose of defining risk and robustness under instance perturbations controlled by metric $\metric$. In that case, we simply write $(\X,\Y,\msr,\C,\H,\metric)$ to include $\metric$.  



\begin{definition}[Nice  classification problems]
 We  call $(\X,\Y,\msr,\C,\H,\metric)$ a \emph{nice} classification problem, if the following two conditions hold:
\begin{enumerate}
    \item $(\X, \metric, \msr)$ is a nice metric probability space.
    \item For every $h \in \H,c \in \C$, their error region $\set{x \in \cX \mid h(x) \neq c(x)}$ is $\msr$-measurable.
\end{enumerate}
The second condition above is satisfied, e.g., if  the set of labels $\cY$ (which is usually finite) is countable,  and for all $y \in \cY, f \in \H \cup \C$, the set $\set{x \in \cX \mid f(x)=y} $ is $\msr$-measurable.
\end{definition}



\subsection{The Concentration Function and Some  Bounds}
We now formally define the (standard) notion of concentration function.
\begin{definition}[Concentration function] \label{def:conc}
Let $(\X, \metric, \msr)$ be a metric probability space and $\cE \se \X$ be a Borel set. 
The \emph{concentration function} is then defined as
    $$ \con(b)= 1-\inf \set{\msr(\cE_b) \mid \msr(\cE) \geq 1/2}.$$
\end{definition}

\begin{definition}[Normal \Levy families] \label{def:Levy}
A  family of  metric probability spaces $(\X_n, \metric_n, \msr_n)_{i\in\N}$ with corresponding concentration functions $\con_n(\cdot)$ is  called a \emph{$(k_1,k_2)$-normal \Levy family}  if 
$$\con_n(b) \leq k_1 \cdot \e^{-k_2\cdot b^2 \cdot n}.$$
When $n$ is clear from the context, we simply write $(\X, \metric, \msr)$ to denote $(\X_n, \metric_n, \msr_n)_{i\in\N}$.
\end{definition}




\begin{lemma}[Concentration of product spaces under Hamming distance]\label{lem:talagrand}
Let $\msr \equiv \msr_1 \times \dots \times \msr_n$ be a product probability measure of dimension $n$ and let  $\HD$ be Hamming distance. For any $\msr$-measurable $\cS \se \X$ such that $\cS_b$ is also measurable, we have
$$\msr(\cS_b) \geq 1- \frac{\e^{-b^2 / n}}{\msr(\cS)} .$$
\end{lemma}

\begin{lemma}[McDiarmid inequality]\label{lem:MCD}
Let  $\msr \equiv \msr_1 \times \dots \times \msr_n$ be a product probability measure of dimension $n$, and let $f\colon \Supp(\msr) \To \R$ be a measurable function such that  $|f(x)-f(y)|\leq 1$ whenever $x$ and $y$  \emph{only} differ in one coordinate. If $a=\Ex_{x \gets \msr}[f(x)]$, then 
$$\Pr_{x \gets \msr}[f(x) \leq a - b] \leq \e^{-2\cdot b^2/n}.$$
%Hoeffding's inequality is special case in which $X_i \in [0,1]$ and $f(X_1,\dots,X_n) = \sum_i X_i$.
\end{lemma}

\begin{lemma}[Azuma's inequality for submartingales] \label{lem:Azuma} Let $\tDistVec \equiv (\tDist_1,\dots,\tDist_n)$ be a sequence of $n$ jointly distributed  random variables such that for all $i \in [n]$, $\Pr[|\tDist_i|> \delta] =0$,  and all $\pfix{t}{i-1}\gets \pfix{\tDist}{i-1}$, it holds that
$\Ex[\tDist_i\mid \pfix{t}{i-1}] \geq 0.$
Then, we have
$$\Pr\left[\sum_{i=1}^n \tDist_i \leq -s\right] \leq \e^{\frac{-s^2}{2n\cdot \delta^2}}.$$
\end{lemma}




The following lemma gives McDiarmid-type inequality starting from a concentration function.
\begin{lemma}[Going from mean to median for Lipcshitz functions using concentration]
Let $f$ be Lipschitz and $a=\Ex_{x \gets \msr}[f(x)]$ and $m$ be the median of $f$. Then, $|m-a| \leq \int_{z=0}^\infty \con(z) \cdot dz$.
\end{lemma}
\begin{proof}
To be written Lemma 3.3 from our previous paper.
\end{proof}

\begin{corollary}[Mean vs. median in normal \Levy families]
Let $(\X, \metric, \msr)$ be a $(k_1,k_2)$-normal \Levy family. Then there is a constant $k_3$ such that  for any Lipschitz function $f$ over $(\X_n,\metric_n)$, if $a=\Ex_{x \gets \msr}[f(x)]$ and $m$ is a median of $f$, then $|m-a|\leq k_3 / \sqrt n$.
\end{corollary}
\begin{proof}
to be written similar to the integral in Theorem 3.7 in previous paper.
\end{proof}


\begin{lemma}[Concentration around mean for normal \Levy families]\label{lem:MCD-Levy}
Let $(\X, \metric, \msr)$ be a $(k_1,k_2)$-normal \Levy family. Then there is a constant $k_3$ such that  for any Lipschitz function $f$ over $(\X_n,\metric_n)$, if $a=\Ex_{x \gets \msr}[f(x)]$ and $b = t + k_3 /\sqrt n$, then 
$$\Pr_{x \gets \msr}[|f(x) - a| \geq b] \leq k_1\e^{-k_2 \cdot t^2 \cdot n}.$$
%Hoeffding's inequality is special case in which $X_i \in [0,1]$ and $f(X_1,\dots,X_n) = \sum_i X_i$.
\end{lemma}
\subsection{Notation and Basic Definitions for Tampering with Random Processes}
\paragraph{Notation.} By $\xDist \equiv \yDist$ we denote that the random variables $\xDist$ and $\yDist$ have the same distributions. Unless stated otherwise, by using a bar over a variable, we emphasize that it is a vector.  By $\xDistVec \equiv (\xDist_1,\xDist_2,\dots,\xDist_n)$ we refer to a joint distribution over vectors with $n$ components.
For a joint distribution $\xDistVec \equiv (\xDist_1,\dots,\xDist_n)$, we use $\pfix{\xDist}{i}$ to denote the joint distribution of the first $i$ variables $\xDistVec \equiv (\xDist_1,\dots,\xDist_i)$. Also, for a vector $\xVec=(x_1\dots x_n)$ we use $\pfix{x}{i}$ to denote the prefix $(x_1,\dots, x_i)$.
%
For a randomized algorithm $L(\cdot)$, by $y \gets L(x)$ we denote the randomized execution of $L$ on input $x$ outputting $y$. For a distribution $(\xDist,\yDist)$, by $(\xDist \mid \yDist)$ we denote the conditional distribution $(\xDist \mid \yDist = y)$. By $\Supp(\xDist) = \set{d \mid \Pr[\xDist=d]>0}$ we denote the support set of $\xDist$. 
By $T^\xDist(\cdot)$ we denote an algorithm $T(\cdot)$ with oracle access to a sampler for distribution $\xDist$ that upon every query returns fresh samples from $\xDist$. By $\xDist \times \yDist$ we refer to the product distribution in which $\xDist$ and $\yDist$ are sampled independently.
By $\xDist^n$ we denote the $n$-fold product $\xDist\times \dots \times \xDist$ returning $n$  iid samples.


%\begin{definition}[Valid prefixes] Let $\xDistVec \equiv (\xDist_1,\dots,\xDist_n)$ be an arbitrary joint distribution. We call $\pfix{x}{i} = (x_1,\dots, x_i)$ a \emph{valid prefix} for $\xDistVec$ if there exist  $x_{i+1},\dots, x_n$ such that $(x_1,\dots, x_n) \in \Supp (\xDistVec)$. $\VP(\xDistVec)$ denotes the set of all valid prefixes of $\xDistVec$. \end{definition}

\paragraph{Tampering attack models.} The following definition defines tampering adversaries who get the first $i$ blocks of an $n$-block sequence, and then decide on the new $i$'th block. Such adversaries can decide not to tamper the $i$'th block by outputting the same block as the current $i$'th one. Previous definitions of tampering adversaries used in \cite{pTampTCC17,Mahloujifar2018:ALT,ITCS-sub} worked with definitions that only give the first $i-1$ first blocks to the adversary and were more general to cover arbitrary random processes that are stateful, but since here we deal with product distributions only, our definition becomes simpler.

\begin{definition} [Online and offline tampering] \label{def:tamp}
 Here we define two attack models and their properties.
\begin{itemize}
    \item {\bf Online attacks.} Let $\xDistVec \equiv \xDist_1\times \dots \times \xDist_n$ be an arbitrary product distribution.\footnote{We restrict the case of online attacks to product distribution as they will have simpler notations and that they cover our main applications, however they can be generalized to arbitrary joint distributions as well with a bit more care.} We call a (potentially randomized and  computationally unbounded) algorithm $\OnlTam$ an  \emph{online tampering} algorithm for $\xDistVec$, if given any $i\in[n]$ and any $\pfix{x}{i} \in \Supp(\xDist_1)\times \dots \times \Supp(\xDist_i)$, it holds that
$$\Pr_{y_i \gets \OnlTam(\pfix{x}{i})}[y_i \in \Supp(\xDist_i)]=1 ~.$$
Namely, $ \OnlTam(\pfix{x}{i})$  outputs (a candidate $i$'th block) $y_i$ that is also in the support set of $\xDist_i$. 
    \item {\bf Offline attacks.} For an arbitrary joint distribution $\xDistVec \equiv (\xDist_1\dots,\xDist_n)$ (that might or might not be a product distribution), we call a (potentially randomized and possibly computationally unbounded) algorithm $\OffTam$ an  \emph{offline tampering} algorithm for $\xDistVec$, if given any  $\xVec \in \Supp(\xDistVec)$, it holds that
$$\Pr_{\yVec \gets \OnlTam(\xVec)}[\yVec \in \Supp(\xDistVec)]=1 ~.$$
Namely, given any $\xVec \gets \xDistVec$, $ \OnlTam(\xVec)$ always outputs a vector  that is also in the support set of $\xDistVec$. 
    \item {\bf Efficiency of attacks.}
We call an online or offline tampering algorithm $\Tam$ \emph{efficient}, if its running time is $\poly(N)$ where $N$ is the total bit length of representing any $\xVec \in \Supp(\xDist)^n$. (Equivalently, it runs in time $\poly(n \cdot D)$ where $D$ is the total bit length of representing any $x \in \Supp(\xDist)$.)\footnote{Fixing $n$ is important for the definition of efficient tampering algorithms, as larger $n$ allows them to run in longer time.}
    \item {\bf Notation for tampered distributions.} For any joint distribution $\xDistVec$, any $\xVec \gets \xDistVec$, and for any tampering algorithm $\Tam$, by $\twist{\xVec}{\Tam}$ we refer to the distribution obtained by running $\Tam$ over $\xVec$, and by $\twist{\xVec}{\Tam}$ we refer to the final distribution by also sampling $\xVec \gets \xDistVec$ at random. More formally:
    \begin{itemize}
        \item  For an offline tampering algorithm $\OffTam$, the distribution $\twist{\xVec}{\OffTam}$ is sampled by simply running $\OffTam$ on the whole $\xVec$ and obtaining the output $(y_1,\dots,y_n) \gets \OffTam(x_1,\dots,x_n)$.
        \item For an online tampering algorithm $\OnlTam$ and input $\xVec=(x_1,\dots,x_n)$ sampled from a \emph{product} distribution $\xDist_1\times \dots \xDist_n$, we obtain the output $(y_1,\dots,y_n)  \gets \twist{\xVec}{\OnTam}  $ \emph{inductively} as follows. For $i \in [i]$, sample $y_i \gets \OnTam(y_1,\dots,y_{i-1},x_i)$.\footnote{By limiting our online attackers to product distributions, we can sample the whole sequence of ``untampered'' values $(x_1,\dots,x_n)$ at the beginning; otherwise, for general random processes in which the distribution of blocks are correlated, we would need to sample $(x_1,\dots,x_n)$ and $(y_1,\dots,y_n)$ \emph{jointly} by sampling $x_i$ \emph{conditioned on} $y_1,\dots,y_{i-1}$.}
    \end{itemize}
      
    \item {\bf Budget of tampering attacks.} Suppose $\metric$ is a metric defined over $\Supp(\xDistVec)$. We say an online or offline tampering algorithm $\Tam$ has \emph{budget} (at most) $b$, if 
    $$\Pr_{\substack{\xVec \gets \xDistVec, \\ \yVec \gets \twist{\xVec}{\Tam}}}[\metric(\xVec,\yVec) \leq b] = 1,$$
    and we say that $\Tam$ has \emph{average} budget (at most) $b$ if
    $$\Ex_{\substack{\xVec \gets \xDistVec, \\ \yVec \gets \twist{\xVec}{\Tam}}}[\metric(\xVec,\yVec)] \leq b.$$
    If no metric  $\metric$ is specified, by default we use Hamming distance over vectors of dimension $n$.
\end{itemize}
\end{definition}

%\begin{definition}[Online samplers] We call $\Samp$ an \emph{online sampler} for $\xDistVec \equiv (\xDist_1,\dots,\xDist_n)$ if for all $\pfix{x}{i-1} \in \VP(\xDistVec)$, $\Samp(n,\pfix{x}{i-1}) \equiv \xDist_i$. Moreover, we call $\xDistVec \equiv (\xDist_1,\dots,\xDist_n)$ \emph{online samplable} if it has an online sampler that runs in time $\poly(N)$ where $N$ is maximum  bit length of any $\xVec \in \Supp(\xDistVec)$. \end{definition}

%\begin{definition} [Notation for distributions obtained from tampering attacks] \label{def:tamperingDist} Let $\xDistVec \equiv (\xDist_1,\dots,\xDist_n)$ be an arbitrary joint distribution and $\OnlTam$ a tampering algorithm for $\xDistVec$. For any subset $S \se [n]$, we define $\yDistVec\equiv \twist{\xDistVec}{\OnlTam}$ to be the be a joint distribution that is the result of online tampering of $\OnlTam$ over set $S$, where $\yDistVec \equiv (\yDist_1,\dots,\yDist_n)$ is sampled  inductively  as follows. For every $i\in[n]$, suppose $ \pfix{y}{i-1}$ is the previously sampled block. If $i \in S$, then the $i\th$ block $\yDist_i$ is generated by the tampering algorithm $\OnlTam( \pfix{y}{i-1})$, and otherwise,  $\yDist_i$ is sampled from  $(\xDist_i \mid \xDist_{i-1} =  \pfix{y}{i-1})$. For any \emph{distribution} $\SDist$ over subsets of $[n]$, by $\twist{\xDistVec}{\OnlTam}$ we denote that random variable that can be sampled by first sampling $S \gets \SDist$ and then sampling $\yVec \gets \twist{\xDistVec}{\OnlTam}$. \end{definition}











==> compRob.tex <==







==> productOff.tex <==

\section{Products are Computationally Concentrated under Hamming Distance (Offline Case)}

\Mnote{We should start from here and see what we can prove, and then define abstract notions based on it.}

For simplicity, the following construction is written for the simper case that $\sqrt n$ is an integer. 

\begin{construction}[LBD re-sampler  for the unit cube under Hamming distance]\label{Cons:LBD_HD}
Given an $x\in [0,1]^n$, sample a $b \in [k\cdot \sqrt{n}]$ with relative weight $\e^{-b/k\cdot\sqrt{ n}}$. Then sample a point $x'$ uniformly from $\Sph_b(x)$.
\end{construction}

\begin{claim} The sampler of \ref{Cons:LBD_HD} is $\frac{2}{k\cdot\sqrt{n}}$-Lipschitz.
\end{claim}
\begin{proof}
let $x$ and $x'$ be such that $\HD(x,x') = 1$. Let $\msr_x \equiv \CentDist(x)$ and $\msr_{x'} \equiv \CentDist(x')$. Let $\cB =  \Ball_{k\sqrt{n}-1}(x)$, $\cS_1 = \Sph_{k\sqrt{n}}(x)$ and $\cS_2 = \Sph_{k\sqrt{n}}(x') \sm (\cS_1\cup \cB)$. Note that we have,
$$\msr_x(\cS_1) = \frac{\e^{-1}}{\sum_{i=0}^{k\cdot\sqrt{n}} \e^{-\frac{i}{k\cdot \sqrt{n}}}} = \frac{1-\e^{-\frac{1}{k\cdot \sqrt{n}}}}{\e-\e^{-\frac{1}{k\cdot \sqrt{n}}}}\leq \frac{1}{k\cdot \sqrt{n} \cdot (\e-1)}.$$
Now, the statistical distance between $\CentDist(x) $ and $ \CentDist(x')$ is equal to
\begin{align*}
    & |\CentDist(x) - \CentDist(x')| \\
    &= \sup_{\cA \se [0,1]^n} \left(\msr_x(\cA) - \msr_{x'}(\cA)\right)\\
                                    & = \sup_{\cA \se [0,1]^n}\left(\msr_x(\cA\cap \cB) - \msr_{x'}(\cA\cap \cB) + \msr_x(\cA\cap \cS_1) - \msr_{x'}(\cA\cap \cS_1) + \msr_x(\cA\cap \cS_2) - \msr_{x'}(\cA\cap \cS_2) )\right)\\
                                    &= \sup_{\cA \se [0,1]^n}\left(\msr_x(\cA\cap \cB) - \msr_{x'}(\cA\cap \cB) + \msr_x(\cA\cap \cS_1) - \msr_{x'}(\cA\cap \cS_1) - \msr_{x'}(\cA\cap \cS_2) )\right)\\
                                    & \leq \sup_{\cA \se [0,1]^n}\left(\msr_x(\cA\cap \cB) - \msr_{x'}(\cA\cap \cB) + \msr_x(\cA\cap \cS_1))\right)\\
                                    &\leq \sup_{\cA \se [0,1]^n}\left(\msr_x(\cA\cap \cB) - \e^{\frac{-1}{k\sqrt{n}}}\msr_{x}(\cA\cap \cB) + \msr_x(\cA\cap \cS_1))\right)\\
                                    &\leq \sup_{\cA \se [0,1]^n}\left(1 - \e^{\frac{-1}{k\sqrt{n}}} + \msr_x(\cA\cap \cS_1))\right)\\
                                    &\leq 1 - \e^{\frac{-1}{k\sqrt{n}}} + \msr_x(\cS_1)\\
                                    &\leq 1 - \e^{\frac{-1}{k\sqrt{n}}} + \frac{1}{k\sqrt{n}\cdot(\e-1)}\\ 
                                    &\leq \frac{2}{k\sqrt{n}}.
\end{align*}
\end{proof}
\begin{claim}
The LBD re-sampler  of \ref{Cons:LBD_HD} is $k\cdot \sqrt{n}$-bounded and has re-randomization factor $1$.
\end{claim}
\begin{proof}
\end{proof}

\begin{corollary}
Let $\cS$ be a subset of the unit cube $[0,1]^n$ with measure $h$. There is an algorithm $A$ that given $x \in \X$, calls LBD re-sampler  of Construction \ref{Cons:LBD_HD}, $\poly(\frac{1}{h})$ times and outputs $A(x)\in \X$ such that
$$\Pr_{\substack{x\gets [0,1]^n\\ x'\gets A(x)}}[x'\in \cS \wedge \metric(x,x')\leq \beta] \geq 1- \e^{  \frac{- h^2k^2}{8}}.$$
\end{corollary}

